A lattice of combinatorial Hopf algebras, Application to binary trees with multiplicities

In a first part, we formalize the construction of combinatorial Hopf algebras from plactic-like monoids using polynomial realizations. Thank to this construction we reveal a lattice structure on those combinatorial Hopf algebras. As an application, we construct a new combinatorial Hopf algebra on binary trees with multiplicities and use it to prove a hook length formula for those trees. Dans une premi\`ere partie, nous formalisons la construction d'alg\`ebres de Hopf combinatoires \`a partir d'une r\'ealisation polynomiale et de mono\"ides de type mono\"ide plaxique. Gr\^ace \`a cette construction, nous mettons \`a jour une structure de treillis sur ces alg\`ebres de Hopf combinatoires. Comme application, nous construisons une nouvelle alg\`ebre de Hopf sur des arbres binaires \`a multiplicit\'es et on l'utilise pour d\'emontrer une formule des \'equerres sur ces arbres.

==> arbres/exSucc/s8.tex <==
\begin{tikzpicture}[every node/.style={draw,circle}]
    \node (0) at (1/1.4,3) {$\scriptstyle 4$};
    \node (2) at (2/1.4,1) {$\scriptstyle 1$};
    \node (1) at (3/1.4,2) {$\scriptstyle 1$};
    \node (3) at (4/1.4,1) {$\scriptstyle 1$};
\path[red,ultra thick]
    (1) edge (2)
    (1) edge (3)
    (0) edge (1)
;\end{tikzpicture}


==> arbres/exSucc/s9.tex <==
\begin{tikzpicture}[every node/.style={draw,circle}]
    \node (1) at (1/1.4,2) {$\scriptstyle 1$};
    \node (0) at (2/1.4,3) {$\scriptstyle 3$};
    \node (2) at (3/1.4,2) {$\scriptstyle 2$};
    \node (3) at (4/1.4,1) {$\scriptstyle 1$};
\path[red,ultra thick]
    (2) edge (3)
    (0) edge (1)
    (0) edge (2)
;\end{tikzpicture}

==> arbres/exSucc/t.tex <==
\begin{tikzpicture}[every node/.style={draw,circle}]
    \node (1) at (1/1.4,2) {$\scriptstyle 1$};
    \node (0) at (2/1.4,3) {$\scriptstyle 3$};
    \node (3) at (3/1.4,1) {$\scriptstyle 1$};
    \node (2) at (4/1.4,2) {$\scriptstyle 1$};
    \node (4) at (5/1.4,1) {$\scriptstyle 1$};
\path[red,ultra thick]
    (2) edge (3)
    (2) edge (4)
    (0) edge (1)
    (0) edge (2)
;\end{tikzpicture}

==> arbres/opeSuccEta.tex <==
\newcommand{\AOnooa}{\node (1) [circle, fill=white, text=black, draw] 
    {$k$};}\newcommand{\AOnoob}{\node (2) [rectangle,fill=orange!80,draw=blue, thick] 
    {};}\newcommand{\AOnooc}{\node (3) [rectangle,fill=orange!80,draw=blue, thick] 
    {$\tau$};}\newcommand{\AOnood}{\node (4) [rectangle,fill=orange!80,draw=blue, thick] 
    {$\sigma$};}\newcommand{\AOnoof}{\node (6) [circle, fill=white, text=black, draw] 
    {$\scriptstyle k-j$};}\newcommand{\AOnoog}{\node (7) [rectangle,fill=orange!80,draw=blue, thick] 
    {};}\newcommand{\AOnooh}{\node (8) [circle, fill=white, text=black, draw] 
    {$j$};}\newcommand{\AOnooi}{\node (9) [rectangle,fill=orange!80,draw=blue, thick] 
    {$\tau$};}\newcommand{\AOnooj}{\node (10) [rectangle,fill=orange!80,draw=blue, thick] 
    {$\sigma$};}\newcommand{\AOnook}{\node (11) [circle, fill=white, text=black, draw] 
    {$\scriptstyle k-j$};}\newcommand{\AOnool}{\node (12) [rectangle,fill=orange!80,draw=blue, thick] 
    {};}\newcommand{\AOnoom}{\node (13) [circle, fill=white, text=black, draw] 
    {$j$};}\newcommand{\AOnoon}{\node (14) [rectangle,fill=orange!80,draw=blue, thick] 
    {$\tau$};}\newcommand{\AOnooo}{\node (15) [rectangle,fill=orange!80,draw=blue, thick] 
    {$\sigma$};}\begin{tikzpicture}[auto]
\matrix[column sep=.1cm, row sep=.5cm]{
             & \AOnooa   &           &&&&         & \AOnoof  &          &         &&&&         & \AOnook\\ 
  \AOnoob    &           &  \AOnooc  &&\node{$\xrightarrow{\eta_{i,j}}$};&& \AOnoog &          & \AOnooh  &         &&\node{and};&& \AOnool &          & \AOnoon    \\
             &           &  \AOnood  &&&&         &          &          & \AOnooi &&&&         & \AOnoom \\
             &           &           &&&&         &          &          & \AOnooj &&&&         &          & \AOnooo\\
};
\path[red, ultra thick] 
    (1) edge (2) edge (3)
    (3) edge[dashed] (4);
\path[red, ultra thick] 
    (6) edge (7) edge (8)
    (8) edge (9)
    (9) edge[dashed] (10);
\path[red, ultra thick] 
    (11) edge (12) edge (14)
    (14) edge[dashed] (13)
    (13) edge[dashed] (15);
\end{tikzpicture}

% \newcommand{\AOnood}{\node (4) [circle, fill=white, text=black, draw] 
%     {$\scriptstyle k-j$};}\newcommand{\AOnooe}{\node (5) [rectangle,fill=orange!80,draw=blue, thick] 
%     {};}\newcommand{\AOnoof}{\node (6) [rectangle,fill=orange!80,draw=blue, thick] 
%     {};}\begin{tikzpicture}[auto]
% \matrix[column sep=.1cm, row sep=.1cm]{
%           & \AOnood\\ 
%  \AOnooe  &\\  
% };
% \path[red, ultra thick] 
%     (4) edge (5);
% \end{tikzpicture}

==> arbres/opeSuccPi.tex <==
\newcommand{\AOnoae}{\node (15) [circle, fill=white, text=black, draw] 
    {$k$};}\newcommand{\AOnoaf}{\node (16) [circle, fill=white, text=black, draw] 
    {$l$};}\newcommand{\AOnoag}{\node (17) [rectangle,fill=orange!80,draw=blue, thick] 
    {};}\newcommand{\AOnoah}{\node (18) [rectangle,fill=orange!80,draw=blue, thick] 
    {$\alpha$};}\newcommand{\AOnoai}{\node (19) [rectangle,fill=orange!80,draw=blue, thick] 
    {$\tau$};}\newcommand{\AOnooa}{\node (20) [circle, fill=white, text=black, draw] 
    {$\scriptstyle k+m$};}\newcommand{\AOnoob}{\node (21) [circle, fill=white, text=black, draw] 
    {$l$};}\newcommand{\AOnooc}{\node (22) [circle, fill=white, text=black, draw] 
    {$m$};}\newcommand{\AOnood}{\node (23) [rectangle,fill=orange!80,draw=blue, thick] 
    {};}\newcommand{\AOnooe}{\node (24) [rectangle,fill=orange!80,draw=blue, thick] 
    {$\tau$};}\begin{tikzpicture}[auto]
\matrix[column sep=.1cm, row sep=.1cm]{
             & \AOnoae   &           & &  &   &          & \AOnooa\\ 
  \AOnoai    &           &  \AOnoag  & & \node{$\xrightarrow{\pi_i}$};  &   & \AOnooe  &           &  \AOnood\\
             & \AOnooc   &           & &  &   &          & \\  
};
\path[red, ultra thick] 
    (15) edge (19) edge (17)
    (19) edge (22)
    (20) edge (24) edge (23);
\end{tikzpicture}

==> arbres/quasiperm.tex <==
Pour construire le pseudo-permutohèdre (treillis des mots tassés), il 
nous faut introduire :
\begin{itemize}
  \item les \emph{inversions} sont les couples de positions $(i,j)$ 
    dans un mot $w$ tels que $i<j$ et $w[i] > w[j]$; et 
  \item les \emph{demi-inversions} sont aussi des couples de positions
    où $i<j$ mais $w[i] = w[j]$. 
\end{itemize} 

\begin{exemple}
    Soient $u := (1121343)$ et $v := (1231413)$ deux mots tassés.
    L'ensemble d'inversions de $u$ est $\{(3,4), (6,7)\}$ et de 
    demi-inversions $\{(1,2),(1,4),(2,4),(5,7)\}$; et pour $v$ 
    l'ensemble d'inversions est $\{(2,4),(2,6),(3,4),(3,6)\}$ et 
    l'ensemble de demi-inversions est $\{(1,4),(1,6),(3,7),(4,6)\}$.
    On a alors $u \preceq v$ car $2 + \frac{1}{2}2 \leqslant 4 + 
    \frac{1}{2}4$.
\end{exemple}
Le pseudo-permutohèdre se construit par la relation d'ordre partielle 
$\preceq$ définit par $u\preceq v$ si pour $(i,j)$ tel que $i<j$
l'inversion de $u$ est inférieure à celle $v$.
Cet ordre partiel forme un treillis \cite{krob2000pseudo}. La relation
de couverture se définit sur les mots tassés comme suit : les 
successeurs de $u$ sont donné par les fonctions $\pi_j$ et $\eta_{i,j}$ :
\begin{itemize}
  \item $\pi_j(u) = (a_1 \ldots a_n)$ est définit s'il existe 
    $i\leqslant j$ tel que toutes les lettres $i-1$ sont à gauche des 
    lettres $i$ alors $a_k = u[k]$ si $u[k]<j$ et $u[k]-1$ sinon,
  \item $\eta_{i,j}(u) = (a_1 \ldots a_n)$ où $a_k = u[k]$ si $u[k] <i$
    ou $u[k]= i$ et $k$ est à droite des $j$ premières occurrences de
    $i$; et, $a_k = u[k]+1$ sinon. 
\end{itemize}

\begin{exemple}
    \begin{sagesilent}
        pw = PackedWord([1,1,4,2,2,3,3])
    \end{sagesilent}
    Les successeurs $v$ du mot tassés $u := \sage{pw}$ ($u \preceq v$) 
    sont les mots de l'ensemble : 
   \[\sage{Set(pw.quasi_permutohedron_succ())}\;.\] 
\end{exemple}

Cet ordre partiel forme un treillis \cite{krob2000pseudo} 
(\textit{cf}. figure \ref{figQuasiPerm}) et celui-ci a la propriété
suivante : 

\begin{thm}
    Le produit des $\MM_u$ de \wqsym forme un intervalle du 
    quasi-permutohèdre :
    \[\MM_u \times \MM_v = \sum_{w \in [u\cdot v^{\uparrow k}, u^{\uparrow l}\cdot v]}\]
    où $k,l$ sont respectivement les lettres maximales de $u$ et $v$ ; et 
    $w^{\uparrow k}$ le mot où chaque lettre de $w$ est décalée de $k$ positions dans 
    l'alphabet.
\end{thm} 
 
\begin{exemple}
    \begin{sagesilent}
        M = WQSym(QQ).M()
    \end{sagesilent}
    \begin{eqnarray*}
        \sage{M[1]} \times \sage{M[1,2]} &=& 
        \sum_{w \in [(123), (312)]} \MM_{w} 
        = \sage{M[1] * M[1,2]}
    \end{eqnarray*}
\end{exemple}

Ce théorème permet notamment de donner des bases multiplicatives à \wqsym. 

==> arbres/quasisylv.tex <==
\begin{lemme}
    Taïga relation (\ref{eqnTaig}) is a lattice congruence for 
    quasi-permutohedron.
    
    We call the lattice obtained \emph{\quasi-sylvestrohedron}.
\end{lemme} 

The covering relation of \emph{\quasi-permutohedron} are easily translated
in \emph{\quasi-sylvestrohedron} as the following. These following two functions  
$\pi_i$ and $\eta_{i,j}$ compute successors of a tree in \quasi-sylvestrohedron:

\begin{minipage}[b]{0.60\linewidth}
    \begin{itemize}
  \item the function $\pi_i$ merges a node with its most right node in 
  its left child;
\end{itemize}
\end{minipage}\hfill
\begin{minipage}[b]{0.35\linewidth}
    \[\vcenter{\hbox{
      \scalebox{.6}{$\input{arbres/opeSuccPi}$}
    }}\]
\end{minipage}

\begin{minipage}[b]{0.60\linewidth}
    \begin{itemize}
  \item the function $\eta_{i,j}$ remove $j$ at the multiplicity of a
    node $n$ such that $k:=m(n)>j$ and insert a new one $n'$ to any position in
    its right child such that it is the smallest node of the right child
    tree such that $m(n')=j$ and $m(n)=k-j$.
\end{itemize}
\end{minipage}\hfill
\begin{minipage}[b]{0.35\linewidth}
    \[\vcenter{\hbox{
      \scalebox{.6}{\input{arbres/opeSuccEta}}
    }}\]
\end{minipage}

\begin{exemple}
    The tree $\vcenter{\hbox{\scalebox{.4}{\input{arbres/exSucc/t}}}}$ 
    has this set of successors: 
    \[\left\{
    \vcenter{\hbox{\scalebox{.4}{\input{arbres/exSucc/s8}}}},
    \vcenter{\hbox{\scalebox{.4}{\input{arbres/exSucc/s9}}}},
    \vcenter{\hbox{\scalebox{.4}{\input{arbres/exSucc/s2}}}},
    \vcenter{\hbox{\scalebox{.4}{\input{arbres/exSucc/s6}}}},
    \vcenter{\hbox{\scalebox{.4}{\input{arbres/exSucc/s4}}}},
    \vcenter{\hbox{\scalebox{.4}{\input{arbres/exSucc/s3}}}},
    \vcenter{\hbox{\scalebox{.4}{\input{arbres/exSucc/s1}}}},
    \vcenter{\hbox{\scalebox{.4}{\input{arbres/exSucc/s5}}}}
    \right\}\]
\end{exemple}

If we interess to projection of multiplicatives bases of \wqsym in 
$\wqsym/_{\equiv_t}$ we remark that bases don't stay multiplicatives.
Another way is to remark product of elements $(\QQ^m_t)_t$ is not 
necessary an interval of \quasi-permutohedron {\small(\textit{ex}:
$\sage{Qm[2,1]}\times \sage{Qm[1]}$ isn't an interval of 
\quasi-sylvestrohedron of size 3 (figure \ref{figQuasiSylv}))}. 
That trick use to build some multiplicatives basis doesn't work here.
Futhermore we could imagine that doesn't work because of the "stalactic
Hopf algebra": projection of multiplicative bases of \wqsym in this
aren't multiplicatives.

An interesting thing could be to study if union of two relations which 
are $\phi$-good congruences and lattice congruences is a sufficiant 
property to build multiplicatives bases. (That hypothesis is verified
on Baxter Hopf algebra \cite{giraudo, giraudo2012algebraic}.)     


==> arbres/quotient/prod/b1.tex <==
{\newcommand{\AOnooo}{\node (0) [shape=rectangle, rounded corners, draw=blue!80, ultra thick] 
{$1$};}\newcommand{\AOnooa}{\node (1) [shape=rectangle, draw=orange!80, ultra thick] 
{$2$};}\newcommand{\AOnoob}{\node (2) [shape=ellipse, draw=c1,ultra thick, decorate, decoration=zigzag] 
{$1$};}\newcommand{\AOnooc}{\node (3) [circle, draw=c3, ultra thick] 
{$1$};}\begin{tikzpicture}[auto]
\matrix[column sep=.1cm, row sep=.1cm]{
 \AOnooc \\ 
                & \AOnooo \\ 
 \AOnooa &                & \AOnoob \\ 
};
\path[red, ultra thick] (0) edge node {} (2);
\path[red, ultra thick] (0) edge node {} (1);
\path[red, ultra thick] (3) edge node {} (0);
\end{tikzpicture}}

==> arbres/quotient/prod/b2.tex <==
{\newcommand{\AOnooo}{\node (0) [shape=rectangle, rounded corners, draw=blue!80, ultra thick] 
{$1$};}\newcommand{\AOnooa}{\node (1) [shape=rectangle, draw=orange!80, ultra thick] 
{$2$};}\newcommand{\AOnoob}{\node (2) [shape=ellipse, draw=c1,ultra thick, decorate, decoration=zigzag] 
{$1$};}\newcommand{\AOnooc}{\node (3) [circle, draw=c3, ultra thick] 
{$\boldsymbol{3}$};}\begin{tikzpicture}[auto]
\matrix[column sep=.1cm, row sep=.1cm]{
 \node[rectangle,draw=orange!80,ultra thick, text=white]{$2$}; \AOnooc\\ 
        & \AOnooo \\ 
        &         & \AOnoob \\ 
};
\path[red, ultra thick] (0) edge node {} (2);
\path[red, ultra thick] (3) edge node {} (0);
\end{tikzpicture}}

==> arbres/quotient/prod/b3.tex <==
{\newcommand{\AOnooo}{\node (0) [shape=rectangle, rounded corners, draw=blue!80, ultra thick] 
{$1$};}\newcommand{\AOnooa}{\node (1) [shape=rectangle, draw=orange!80, ultra thick] 
{$2$};}\newcommand{\AOnoob}{\node (2) [shape=ellipse, draw=c1,ultra thick, decorate, decoration=zigzag] 
{$1$};}\newcommand{\AOnooc}{\node (3) [circle, draw=c3, ultra thick] 
{$1$};}\begin{tikzpicture}[auto]
\matrix[column sep=.1cm, row sep=.1cm]{
        & \AOnooc\\ 
\AOnooa &         & \AOnooo \\ 
        &         &         & \AOnoob \\ 
};
\path[red, ultra thick] (3) edge (1) edge (0)
                        (0) edge (2);
\end{tikzpicture}}

==> arbres/quotient/prod/b4.tex <==
{\newcommand{\AOnooo}{\node (0) [shape=rectangle, rounded corners, draw=blue!80, ultra thick] 
{$1$};}\newcommand{\AOnooa}{\node (1) [shape=rectangle, draw=orange!80, ultra thick] 
{$2$};}\newcommand{\AOnoob}{\node (2) [shape=ellipse, draw=c1,ultra thick, decorate, decoration=zigzag] 
{$1$};}\newcommand{\AOnooc}{\node (3) [circle, draw=c3, ultra thick] 
{$\boldsymbol{2}$};}\begin{tikzpicture}[auto]
\matrix[column sep=.1cm, row sep=.1cm]{
        & \node[shape=rectangle, rounded corners, draw=blue!80, ultra thick,text=white]{1};\AOnooc\\ 
\AOnooa &         & \AOnoob \\  
};
\path[red, ultra thick] (3) edge (1) edge (2);
\end{tikzpicture}}

==> arbres/quotient/prod/b5.tex <==
{\newcommand{\AOnooo}{\node (0) [shape=rectangle, rounded corners, draw=blue!80, ultra thick] 
{$1$};}\newcommand{\AOnooa}{\node (1) [shape=rectangle, draw=orange!80, ultra thick] 
{$2$};}\newcommand{\AOnoob}{\node (2) [shape=ellipse, draw=c1,ultra thick, decorate, decoration=zigzag] 
{$1$};}\newcommand{\AOnooc}{\node (3) [circle, draw=c3, ultra thick] 
{$1$};}\begin{tikzpicture}[auto]
\matrix[column sep=.1cm, row sep=.1cm]{
        &         & \AOnooc \\ 
        & \AOnooo &         & \AOnoob \\ 
\AOnooa \\ 
};
\path[red, ultra thick] (3) edge (0) edge (2)
                        (0) edge (1);
\end{tikzpicture}}

==> arbres/quotient/prod/b6.tex <==
{\newcommand{\AOnooo}{\node (0) [shape=rectangle, rounded corners, draw=blue!80, ultra thick] 
{$1$};}\newcommand{\AOnooa}{\node (1) [shape=rectangle, draw=orange!80, ultra thick] 
{$2$};}\newcommand{\AOnoob}{\node (2) [shape=ellipse, draw=c1,ultra thick, decorate, decoration=zigzag] 
{$1$};}\newcommand{\AOnooc}{\node (3) [circle, draw=c3, ultra thick] 
{$\boldsymbol{2}$};}\begin{tikzpicture}[auto]
\matrix[column sep=.1cm, row sep=.1cm]{
        &         & \node[text=white, shape=ellipse, draw=c1,ultra thick, decorate, decoration=zigzag]{1};\AOnooc \\ 
        & \AOnooo \\ 
\AOnooa \\ 
};
\path[red, ultra thick] (3) edge (0) 
                        (0) edge (1);
\end{tikzpicture}}

==> arbres/quotient/prod/b7.tex <==
{\newcommand{\AOnooo}{\node (0) [shape=rectangle, rounded corners, draw=blue!80, ultra thick] 
{$1$};}\newcommand{\AOnooa}{\node (1) [shape=rectangle, draw=orange!80, ultra thick] 
{$2$};}\newcommand{\AOnoob}{\node (2) [shape=ellipse, draw=c1,ultra thick, decorate, decoration=zigzag] 
{$1$};}\newcommand{\AOnooc}{\node (3) [circle, draw=c3, ultra thick] 
{$1$};}\begin{tikzpicture}[auto]
\matrix[column sep=.1cm, row sep=.1cm]{
        &         & \AOnooc \\ 
        & \AOnooo \\ 
\AOnooa &         & \AOnoob \\ 
};
\path[red, ultra thick] (3) edge (0)
                        (0) edge (1) edge (2);
\end{tikzpicture}}

==> arbres/sylv.tex <==
In \pbt, the product of $\PP_t$ describes an interval of lattice quotient of
permutohedron: sylvestrohedron \cite{hivert2005algebra}.
Similarly, in \pbtm  the product of $\QQ^m_t$ describes
an interval of a \quasi-permutohedron \cite{krob2000pseudo,
novelli605061polynomial} quotient.

\begin{figure}[H]
%\[\hbox to 0pt {\hss\begin{tabular}{cc}
\begin{minipage}[b]{0.47\linewidth}
    \[\vcenter{\hbox{\scalebox{1}{\input{arbres/sylv2}}}}\] 
    \caption{\label{figQuasiPerm}Quasi-permutohedron of packed words of size 3.}
\end{minipage}\hfill
\begin{minipage}[b]{0.47\linewidth}
    \[\vcenter{\hbox{\scalebox{.38}{\input{arbres/sylv1}}}}\]
    \caption{\label{figQuasiSylv}Quasi-sylvestrohedron of binary tree 
    of non-negative integers of size 3. This lattice is a quotient 
    of quasi-permutohedron figure \ref{figQuasiPerm}.}
\end{minipage} 
\end{figure}
% \subsubsection{Quasi-permutohèdre}     \input{arbres/quasiperm}
% \subsubsection{Quasi-sylvestrohèdron}  
\input{arbres/quasisylv}

==> arbres/sylv1.tex <==
\begin{tikzpicture}[auto,on grid, node distance=2.5cm]
    \node[matrix](123) {
       & & \node[circle, draw](123-r1) {1};\\
       & \node[circle, draw](123-r2) {1};\\
       \node[circle, draw](123-r3) {1};\\
    };
    \path[ultra thick, red] (123-r2) edge (123-r1) edge (123-r3);
    
    \node[matrix](112) [below right=of 123]{
       & \node[circle, draw](112-r1) {1};\\
       \node[circle, draw](112-r2) {2};\\
    };
    \path[ultra thick, red] (112-r2) edge (112-r1);
    
    \node[matrix](213) [below=of 112]{
       & \node[circle, draw](213-r1) {1};\\
       \node[circle, draw](213-r2) {1};\\
       & \node[circle, draw](213-r3) {1};\\
    };
    \path[ultra thick, red] (213-r2) edge (213-r1) edge (213-r3);
    
    \node[matrix](122) [below left=of 213]{
       & \node[circle, draw](122-r1) {2};\\
       \node[circle, draw](122-r2) {1};\\
    };
    \path[ultra thick, red] (122-r2) edge (122-r1);
    
    \node[matrix](132) [below left=of 122]{
       & \node[circle, draw](132-r1) {1};\\
       \node[circle, draw](132-r2) {1}; & & \node[circle, draw](132-r3) {1};\\
    };
    \path[ultra thick, red] (132-r1) edge (132-r2) edge (132-r3);
    
    \node[matrix](111) [below right=of 122]{
       & \node[circle, draw](111-r1) {3};\\
    }; 
    
    \node[matrix](211) [below right=of 132]{
       \node[circle, draw](211-r1) {2};\\
       &\node[circle, draw](211-r2) {1};\\
    };
    \path[ultra thick, red] (211-r1) edge (211-r2);
    
    \node[matrix](231) [below=of 211]{
       \node[circle, draw](231-r1) {1};\\
       &\node[circle, draw](231-r2) {1};\\
       \node[circle, draw](231-r3) {1};\\
    };
    \path[ultra thick, red] (231-r2) edge (231-r1) edge (231-r3);
    
    \node[matrix](221) [below right=of 231]{
       \node[circle, draw](221-r1) {1};\\
       &\node[circle, draw](221-r2) {2};\\
    };
    \path[ultra thick, red] (221-r1) edge (221-r2);
    
    \node[matrix](321) [below=of 221]{
       \node[circle, draw](321-r1) {1};\\
       &\node[circle, draw](321-r2) {1};\\
       & &\node[circle, draw](321-r3) {1};\\
    };
    \path[ultra thick, red] (321-r2) edge (321-r3) edge (321-r1);
    
    \path[ultra thick, blue] (123) edge (112) edge (122)
                             (112) edge (213) edge[bend left=45] (111)
                             (213) edge (122)
                             (122) edge (111) edge (132)
                             (111) edge (211) edge (221)
                             (132) edge (211)
                             (211) edge (231) edge[bend right=60] (321)
                             (231) edge (221)
                             (221) edge (321);
\end{tikzpicture}

==> arbres/sylv2.tex <==
{\newcommand{\AOnooa}{\node (1) [rectangle, fill=white, text=black] 
{$(123)$};}\newcommand{\AOnoob}{\node (2) [rectangle, fill=white, text=black] 
{$(112)$};}\newcommand{\AOnooc}{\node (3) [rectangle, fill=white, text=black] 
{$(122)$};}\newcommand{\AOnood}{\node (4) [rectangle, fill=white, text=black] 
{$(213)$};}\newcommand{\AOnooe}{\node (5) [rectangle, fill=white, text=black] 
{$(132)$};}\newcommand{\AOnoof}{\node (6) [rectangle, fill=white, text=black] 
{$(212)$};}\newcommand{\AOnoog}{\node (7) [rectangle, fill=white, text=black] 
{$(121)$};}\newcommand{\AOnooh}{\node (8) [rectangle, fill=white, text=black] 
{$(111)$};}\newcommand{\AOnooi}{\node (9) [rectangle, fill=white, text=black] 
{$(312)$};}\newcommand{\AOnoao}{\node (10) [rectangle, fill=white, text=black] 
{$(231)$};}\newcommand{\AOnoaa}{\node (11) [rectangle, fill=white, text=black] 
{$(211)$};}\newcommand{\AOnoab}{\node (12) [rectangle, fill=white, text=black] 
{$(221)$};}\newcommand{\AOnoac}{\node (13) [rectangle, fill=white, text=black] 
{$(321)$};}\begin{tikzpicture}[auto]
\matrix[column sep=.1cm, row sep=.5cm]{
                &                & \AOnooa \\ 
                & \AOnoob &                & \AOnooc \\ 
 \AOnood &                &                &                & \AOnooe \\ 
 \AOnoof &                & \AOnooh &                & \AOnoog \\ 
 \AOnooi &                &                &                & \AOnoao \\ 
                & \AOnoaa &                & \AOnoab \\ 
                &                & \AOnoac \\ 
};
\path[blue, ultra thick] (10) edge node {} (12);
\path[blue, ultra thick] (1) edge node {} (2);
\path[blue, ultra thick] (5) edge node {} (7);
\path[blue, ultra thick] (2) edge node {} (4);
\path[blue, ultra thick] (3) edge node {} (5);
\path[blue, ultra thick] (11) edge node {} (13);
\path[blue, ultra thick] (3) edge node {} (8);
\path[blue, ultra thick] (8) edge node {} (11);
\path[blue, ultra thick] (7) edge node {} (10);
\path[blue, ultra thick] (4) edge node {} (6);
\path[blue, ultra thick] (6) edge node {} (9);
\path[blue, ultra thick] (1) edge node {} (3);
\path[blue, ultra thick] (8) edge node {} (12);
\path[blue, ultra thick] (12) edge node {} (13);
\path[blue, ultra thick] (2) edge node {} (8);
\path[blue, ultra thick] (9) edge node {} (11);
\end{tikzpicture}}

==> bon_mono/exStal/a1.tex <==
% pi (112)
\begin{tikzpicture}[scale=.3]
    \foreach \x in {0,-1} {
        \draw (0,\x) rectangle (1,\x + 1);
        \draw (.5,\x+.5) node{$\scriptstyle 1$};
    }
    \foreach \x in {0} {
        \draw (1,\x) rectangle (2,\x + 1);
        \draw (1.5,\x+.5) node{$\scriptstyle 2$};
    }
\end{tikzpicture}

==> bon_mono/exStal/a2.tex <==
% pi (11)
\begin{tikzpicture}[scale=.3]
    \foreach \x in {0,-1} {
        \draw (0,\x) rectangle (1,\x + 1);
        \draw (.5,\x+.5) node{$\scriptstyle 1$};
    }
\end{tikzpicture}

==> defi/a.tex <==
\subsection{Notations}
    \input{defi/notation}

\subsection{Bonnes algèbres}
    \input{defi/bonne_alg}

\subsection{Bons monoïdes}
%     \input{defi/bons_mono}

==> defi/bonne_alg.tex <==
La notion de \emph{bonne algèbre de Hopf} va permettre de généraliser la notion 
de \emph{bon monoïde} introduite par \nom{Hivert-Nzeutchap}\cite{hivert5combinatoire,
hivertnzeutchap2007}.

\begin{defi}[Bonne algèbre de Hopf]
	Soit $\H$ une algèbre de Hopf, et $(B_i)_i$ une de ces bases.
	L'algèbre de Hopf $\H$ est une \emph{bonne algèbre de Hopf} si 
	\begin{itemize}
	  \item le produit des $B_i$ s'exprime comme le \emph{produit de concaténation} 
	  	sur les mots par \emph{réalisation polynomiale},
	  \item et, le coproduit des $B_i$ se définit dans l'algèbre libre par
	  	\emph{doublement d'alphabet}.
	\end{itemize}
	
	On notera $\phi$ la fonction associant à un mot du monoïde libre, un indice $i$
	de $(B_i)_i$ dans la réalisation polynomiale. (On dira que $\phi$ est
	une \emph{bonne fonction} associée à $\H$.)
\end{defi}

Typiquement une \emph{bonne algèbre} va désigner \fqsym\cite{duchamp2001noncommutative,
malvenuto1995duality}, \wqsym \cite{hivert1999combinatoire, bergeron2005hopf, 
novelli2005construction} et \pqsym \cite{novelli2003hopf}, et $\phi$ respectivement 
la fonction de \emph{standardisation}, \emph{tassement} ou \emph{parkisation}.
De plus, les $i$ indicant les éléments $B_i$ de l'algèbre sont les respectivement dans
ces cas les \emph{permutations}, \emph{partitions ordonnées d'ensembles} ou 
\emph{mots tassés} et \emph{fonctions de parking}. 

==> defi/notation.tex <==
Tout au long de l'article nous noterons $\Ag$ un \emph{alphabet infini 
totalement ordonné}. Cet alphabet donne la base du \emph{monoïde libre} $\Ag^*$ 
et sur lequel on définit l'\emph{algèbre libre} $\KA$.
On appelera \emph{somme ordinale} : $\Ag\oplus\Bg$ le monoïde libre 
construit à partir de l'union disjointe de $\Ag$ et $\Bg$ tel que $\forall(a,b) 
\in \Ag \times \Bg$, $a<b$ ; et où pour tout mot, les lettres de $\Ag$ commutent 
avec celles de $\Bg$. 
La notion de somme ordinale sera utilisé avec la notion de \emph{restriction} de 
$w$ à (l'intervalle) $\Cg$ : $w_{|\Cg}$ le plus long sous-mot de $w$ sur 
l'alphabet $\Cg$.


==> header.tex <==
\pagestart{1}

\pageend{14}
\authorhead{J.-B. \textsc  {Priez}\xspace  }
\titlehead{Lattice of combinatorial Hopf algebras, trees with multiplicities}
\titlelong{A lattice of combinatorial Hopf algebras,\\ {\relax \fontsize  {17.28}{22}\selectfont  Application to binary trees with multiplicities.}}
\keywords{Combinatorial Hopf algebras, monoids, polynomial realization, hook length formula, generating series, binary trees}


